Boundary effects on quantum q-breathers in a Bose-Hubbard chain

We investigate the spectrum and eigenstates of a Bose-Hubbard chain containing two bosons with fixed boundary conditions. In the noninteracting case the eigenstates of the system define a two-dimensional normal-mode space. For the interacting case weight functions of the eigenstates are computed by perturbation theory and numerical diagonalization. We identify paths in the two-dimensional normal-mode space which are rims for the weight functions. The decay along and off the rims is algebraic. Intersection of two paths (rims) leads to a local enhancement of the weight functions. We analyze nonperturbative effects due to the degeneracies and the formation of two-boson bound states.

==> elsarticle-template-num.tex <==
<NOSCRIPT>
<META HTTP-EQUIV="Refresh" CONTENT="0;URL=/framework_home/NoScript.html">
</NOSCRIPT>
<!DOCTYPE HTML PUBLIC "-//W3C//DTD HTML 4.01//EN">







 <html><head>
	<title>Elsevier</title>
	<meta http-equiv="imagetoolbar" content="no">
	<meta http-equiv="Content-Style-Type" content="text/css">

	<script language="JavaScript" type="text/javascript">
	<!--
		javascriptLoaderVersion = 5
	// --> 
	</script>

	<link rel="stylesheet" href="/authored_framework/include/css/elsevier.css" type="text/css">
	<link rel="stylesheet" href="/authored_framework/include/css/elsevier2.css" type="text/css">
	<link rel="stylesheet" href="/authored_framework/include/css/v5/menu_ns.css" type="text/css">
	<link rel="stylesheet" href="/authored_framework/include/css/v5/menu_ns2.css" type="text/css">
	<link rel="stylesheet" href="/authored_framework/include/css/v5/menu.css" type="text/css">
	<link rel="stylesheet" href="/authored_framework/include/css/v5/menu2.css" type="text/css">
	<link rel="shortcut icon" href="/favicon.ico" type="image/x-icon" />
	
	<script language="JavaScript" src="/authored_framework/include/js/javascriptLoader.js" type="text/javascript"></script>
	<script language="JavaScript" src="/framework_home/mission.js" type="text/javascript"></script>
	<script language="JavaScript" type="text/javascript">
	<!--

		onload_add(initTopBar)
		if(is.ns4)
			onresize = netscapeRefresh
		else
			onresize = replaceTopBar

		function initTopBar() {
			DynLayerInit();
			replaceTopBar();
			stripNewLine();
		}

		function replaceTopBar() {
			var winWidth = (is.ns)? window.innerWidth:document.body.clientWidth
			if(is.ns5) {
				var xTagLine = winWidth - 530
				var xSearchBox = winWidth - 332
			}
			else if(is.ns4) {
				var xTagLine = winWidth - 530
				var xSearchBox = winWidth - 335
			}
			else {
				var xTagLine = winWidth - 515
				var xSearchBox = winWidth - 318
			}

			if(xTagLine <= 419) xTagLine = 419
			tagLine.moveTo(xTagLine,null)
			topSearchBox.moveTo(xSearchBox,null)
			topSearchBox.show()
		}
		function stripNewLine(){
			if (eval(document.forms[1])){
				if (eval(document.forms[1].address)){
					var str = document.forms[1].address.value;
					if(str!=null){
						if (str.indexOf("\r\n")>-1){
							while (str.indexOf("\r\n")>-1){
								str = str.substr(0,str.indexOf("\r\n")) +"\n" +str.substr(str.indexOf("\r\n")+4);
							}
							document.forms[1].address.value = str;
						}
					}
				}
			}
		}


		function netscapeRefresh() {
			location.href = location.href
		}
	//-->
	</script>
</head>
<body bgcolor="#ffffff" marginwidth="0" leftmargin="0" marginheight="0" topmargin="0"><!-- start of banner -->

<script language="JavaScript" type="text/javascript">
<!--
/*
function changeSearchRadioButtons(form, action) {
	
	form.action.value = action;
}
*/
function submitSearchForm(form) {

	form.submit()

}

function selectSemiRandomImage() {

	var now = new Date();
	var second = now.getSeconds();
	var selectedImage = "/authored_framework/" + "images/topbar_1.jpg";
	
	if (second > 0 && second <= 9) {
		selectedImage = "/authored_framework/" + "images/topbar_1.jpg"; 
	} else if (second > 9 && second <= 19) {
		selectedImage = "/authored_framework/" + "images/topbar_2.jpg";
	} else if (second > 19 && second <= 29) {
		selectedImage = "/authored_framework/" + "images/topbar_3.jpg";
	} else if (second > 29 && second <= 39) {
		selectedImage = "/authored_framework/" + "images/topbar_4.jpg";
	} else if (second > 39 && second <= 49) {
		selectedImage = "/authored_framework/" + "images/topbar_5.jpg";
	} else if (second > 49 && second <= 59) {
		selectedImage = "/authored_framework/" + "images/topbar_6.jpg";
	}
	return selectedImage;
} // end of function

function picswapper(name, images, ms) {
// don't attempt DOM based stuff if the browser isn't DOM compliant. This specifically excludes IE4.
		if (document.getElementById) {
			var name_i = name + '_i'
			var name_images = name + '_images'
			eval(name_i + ' = 0')
			eval(name_images + ' = images')
			eval('document.getElementById("' + name + '").src = ' + name_images + '[0]')
			var code = 'document.getElementById("' + name + '").src = ' + name_images + '[' + name_i + '++ % ' + name_images + '.length]'
			window.setInterval(code, ms)
	}
}
// --> 

var dom = (document.getElementById) ? true : false; 
var ns5 = ((navigator.userAgent.indexOf("Gecko")>-1) && dom) ? true: false; 
var ie5 = ((navigator.userAgent.indexOf("MSIE")>-1) && dom) ? true : false; 
var ns4 = (document.layers && !dom) ? true : false; 
var ie4 = (document.all && !dom) ? true : false; 
var nodyn = (!ns5 && !ns4 && !ie4 && !ie5) ? true : false; 


var origWidth, origHeight; 
if (ns4) { 
 origWidth = window.innerWidth; origHeight = window.innerHeight; 
 window.onresize = function() { if (window.innerWidth != origWidth || window.innerHeight != origHeight) history.go(0); } 
} 

if (nodyn) { event = "nope" } 

var tipFollowMouse= true;
var tipWidth= 360; 
var offX= 20; // how far from mouse to show tip 
var offY= 12; 
//var tipFontFamily= "Verdana, arial, helvetica, sans-serif"; 
var tipFontFamily= "arial"; 
var tipFontSize= "8pt"; 
var tipFontColor= "#000000"; 
var tipBgColor= "#FFFFCC"; 
var tipBorderColor= "#666666"; 
var tipBorderWidth= 1; 
var tipBorderStyle= "outset"; 
var tipPadding= 4; 

var startStr = '<table width="' + tipWidth + '"><tr><td align="center" width="100%">'; 
var midStr = '</td></tr><tr><td valign="top">'; 
var endStr = '</td></tr></table>'; 

var tooltip, tipcss; 
function initMiss() { 


 if (nodyn) return; 
 tooltip = (ns4)? document.tipDiv.document: (ie4)? document.all['tipDiv']: (ie5||ns5)? document.getElementById('tipDiv'): null; 
tipcss = (ns4)? document.tipDiv: tooltip.style; 
if (ie4||ie5||ns5) { 
  tipcss.width = tipWidth+"px"; 
  tipcss.fontFamily = tipFontFamily; 
  tipcss.fontSize = tipFontSize; 
  tipcss.color = tipFontColor; 
  tipcss.backgroundColor = tipBgColor; 
  tipcss.borderColor = tipBorderColor; 
  tipcss.borderWidth = tipBorderWidth+"px"; 
  tipcss.padding = tipPadding+"px"; 
  tipcss.borderStyle = tipBorderStyle; 
 } 
if (tooltip&&tipFollowMouse) { 
  if (ns4) document.captureEvents(Event.MOUSEMOVE); 
 // document.onmousemove = trackMouse; 
 // document.images["mission"].onmousemove = trackMouse; 
 // document.images["mission_two"].onmousemove = trackMouse; 
 } 
} 

//window.onload = initMiss; 

var t1,t2;
var tipOn = false;
function doTooltip(evt,num) { 

 initMiss();
 if (!tooltip) return; 
 if (t1) clearTimeout(t1); if (t2) clearTimeout(t2); 
 tipOn = true; 
 // set colors if included in messages array 
 if (messages[num][2]) var curBgColor = messages[num][2]; 
 else curBgColor = tipBgColor; 
 if (messages[num][3]) var curFontColor = messages[num][3]; 
 else curFontColor = tipFontColor; 
 if (ns4) { 
  var tip = '<table bgcolor="' + tipBorderColor + '" width="' + tipWidth + '" cellspacing="0" cellpadding="' + tipBorderWidth + '" border="0"><tr><td><table bgcolor="' + curBgColor + '" width="100%" cellspacing="0" cellpadding="' + tipPadding + '" border="0"><tr><td>'+ startStr +  midStr + '<span style="font-family:' + tipFontFamily + '; font-size:' + tipFontSize + '; color:' + curFontColor + ';">' + messages[num][1] + '</span>' + endStr + '</td></tr></table></td></tr></table>'; 
  tooltip.write(tip); 
  tooltip.close(); 
 } else if (ie4||ie5||ns5) { 
  var tip = startStr  + midStr + '<span style="font-family:' + tipFontFamily + '; font-size:' + tipFontSize + '; color:' + curFontColor + ';">' + messages[num][1] + '</span>' + endStr; 
  tipcss.backgroundColor = curBgColor; 
   tooltip.innerHTML = tip; 
 } 
 //if (!tipFollowMouse) 
 positionTip(evt); 
 //else
 //t1=setTimeout("tipcss.visibility='visible'",100); 
} 

var mouseX, mouseY; 
function trackMouse(evt) { 

	mouseX = (ns4||ns5)? evt.pageX: window.event.clientX + document.body.scrollLeft; 
 	mouseY = (ns4||ns5)? evt.pageY: window.event.clientY + document.body.scrollTop; 
 	if (tipOn) positionTip(evt); 

} 

function positionTip(evt) { 
 //if (!tipFollowMouse) { 
  mouseX = (ns4||ns5)? evt.pageX: window.event.clientX + document.body.scrollLeft; 
  mouseY = (ns4||ns5)? evt.pageY: window.event.clientY + document.body.scrollTop; 
// } 
 
 // tooltip width and height 
 var tpWd = (ns4)? tooltip.width: (ie4||ie5)? tooltip.clientWidth: tooltip.offsetWidth; 
 var tpHt = (ns4)? tooltip.height: (ie4||ie5)? tooltip.clientHeight: tooltip.offsetHeight; 
 // document area in view (subtract scrollbar width for ns) 
 var winWd = (ns4||ns5)? window.innerWidth-20+window.pageXOffset: document.body.clientWidth+document.body.scrollLeft; 
 var winHt = (ns4||ns5)? window.innerHeight-20+window.pageYOffset: document.body.clientHeight+document.body.scrollTop; 
 // check mouse position against tip and window dimensions 
 // and position the tooltip 
 if ((mouseX+offX+tpWd)>winWd) 
  //tipcss.left = (ns4)? mouseX-(tpWd+offX): mouseX-(tpWd+offX)+"px"; 
   tipcss.left = (ns4)? 179: 179+"px"; 
 else 
 	//tipcss.left = (ns4)? mouseX+offX: mouseX+offX+"px"; 
 	 tipcss.left = (ns4)? 179: 179+"px"; 
 if ((mouseY+offY+tpHt)>winHt) 
   //tipcss.top = (ns4)? winHt-(tpHt+offY): winHt-(tpHt+offY)+"px"; 
   tipcss.top = (ns4)? 125: 125+"px"; 
 else 
   // tipcss.top = (ns4)? mouseY+offY: mouseY+offY+"px"; 
   tipcss.top = (ns4)? 125: 125+"px"; 
 
 //if (!tipFollowMouse)
  t1=setTimeout("tipcss.visibility='visible'",100); 
} 

function hideTip() { 
 if (!tooltip) return; 
 
 t2=setTimeout("tipcss.visibility='hidden'",100); 
 tipOn = false; 

} 


</script>
<div id="tipDiv" style="position:absolute; visibility:hidden; z-index:100"></div>

	<div id="logoDiv">
	<!--Added alerts link on banner part, for PT 1821--> 
		<DIV id=logoDivInner class=verdana10White style="Z-INDEX: 1; LEFT: 0px; WIDTH: 300px; POSITION: absolute; TOP: 105px; HEIGHT: 18px">
		&nbsp;<A href="/wps/find/homepage.cws_home">Home</A> | <A href="/wps/find/sitemap.cws_home/sitemap">Site map</A> | <A href="/wps/find/elsevierwebsites.cws_home/elsevierwebsites">Elsevier websites</A> | <A href="/wps/find/home_content.cws_home/alertingservices">Alerts</A>
		</DIV>
		<img name="mission" src="/authored_framework/images/bg_logo.gif" width="441" height="121" border="0" onmouseover="doTooltip(event,0)" onmouseout="hideTip()"/>
	</div>

	<div id="tagLineDiv">
		<img name="mission_two" src="/authored_framework/images/tagLine.gif" width="192" height="38" border="0" onmouseover="doTooltip(event,0)" onmouseout="hideTip()" />
	</div>

	<div id="topSearchBoxDiv">
		<table cellpadding="0" cellspacing="0" border="0" width="316">
			<tr>
				<td colspan="5" height="1"></td>
			</tr>
			<tr>
				<td bgcolor="#ffffff"><img src="/authored_framework/images/empty.gif" width="1" height="121" border="0" alt="" /></td>

				<td>
					<img id='picswap' src="/authored_framework/images/topbar_1.jpg" width="157" height="121" border="0" alt="Elsevier" />
					<script>
						document.getElementById("picswap").src = selectSemiRandomImage()
					</script>
				</td>
				
				<!-- <td><img id='picswap' src="/authored_framework/images/topbar_1.jpg" width="157" height="121" border="0" alt="Elsevier" />
					<script>picswapper("picswap", [/authored_framework/ + "images/topbar_1.jpg", /authored_framework/ + "images/topbar_2.jpg", /authored_framework/ + "images/topbar_3.jpg", /authored_framework/ + "images/topbar_4.jpg", /authored_framework/ + "images/topbar_5.jpg", /authored_framework/ + "images/topbar_6.jpg"], 5000)</script>
				</td> -->
				
				<td bgcolor="#ffffff"><img src="/authored_framework/images/empty.gif" width="1" height="121" border="0" alt="" /></td>
				<td bgcolor="#ff9933">

<!-- start of search -->

<table cellpadding="0" cellspacing="0" border="0" width="157">
<form NAME="searchForm" METHOD="get" ACTION="/wps/find/simple_search.cws_home" onsubmit="submitSearchForm(document.forms['searchForm']);return false;">
<!--<INPUT TYPE="HIDDEN" NAME="action" VALUE="product_search"/>-->
<INPUT TYPE="HIDDEN" NAME="pubtype" VALUE="Any"/>
<INPUT TYPE="HIDDEN" NAME="boost" VALUE="true"/>
<input TYPE="HIDDEN" NAME="needs_keyword" VALUE="true">
<input TYPE="HIDDEN" NAME="adv" VALUE="false">

<tr>
<td colspan="3"><img src="/authored_framework/images/empty.gif" width="1" height="2" border="0" alt="" /></td>
</tr>
<tr>

<td colspan="3" nowrap="nowrap" align="center">
<!-- <img src="/authored_framework/images/empty.gif" width="4" height="1" border="0" alt="" /> -->
<input type="text" name="keywords" class="searchBox2" tabindex="500" size="15" value="" /></td>
<!-- <td><img src="/authored_framework/images/empty.gif" width="6" height="1" border="0" alt="" /></td> -->
</tr>
<tr>
<td colspan="3"><img src="/authored_framework/images/empty.gif" width="1" height="5" border="0" alt="" /></td>
</tr>
<tr>


<td><input type="radio" name="action" value="product_search" 

	checked="checked"

/></td>


<td><img src="/authored_framework/images/product_info_search.gif" width="110" height="9" border="0" alt="Product information search" /></td>
<td><img src="/authored_framework/images/empty.gif" width="6" height="1" border="0" alt="" /></td>
</tr>
<!--
<tr>
<td colspan="3"><img src="/authored_framework/images/empty.gif" width="1" height="3" border="0" alt="" /></td>
</tr>
-->
<tr>


<td valign="top"><input type="radio" name="action" value="simple_search"

/></td>

<td><img src="/authored_framework/images/all_elsevier_sites_search.gif" width="91" height="9" border="0" alt="Search all Elsevier sites" /></td>
<td><img src="/authored_framework/images/empty.gif" width="6" height="1" border="0" alt="" /></td>
</tr>
<tr>
<td colspan="3"><img src="/authored_framework/images/empty.gif" width="1" height="5" border="0" alt="" /></td>
</tr>
<tr>
<td colspan="2" align="left"><img src="/authored_framework/images/empty.gif" width="3" height="1" border="0" alt="" />
<a href="javascript:submitSearchForm(document.forms['searchForm'])"><img src="/authored_framework/images/banner_search_button.gif" width="58" height="18" border="0" alt="Search" /></a></td>
<td><img src="/authored_framework/images/empty.gif" width="6" height="1" border="0" alt="" /></td>
</tr>
<tr>
<td colspan="3">
<img src="/authored_framework/images/empty.gif" width="3" height="1" border="0" alt="" />
<a href="/wps/find/advproductsearch.cws_home?action=product_search&search=no" class="verdana10DarkGrey">Advanced Product Search</a>
</td>
</tr>
</form>
</table>

<!-- end of search -->

				</td>
				<td bgcolor="#ffffff"><img src="/authored_framework/images/empty.gif" width="2" height="121" border="0" alt="" /></td>
			</tr>
		</table>
	</div>

	<table background="/authored_framework/images/bg.gif" cellpadding="0" cellspacing="0" border="0" width="100%">
		<tr>
			<td style="width:178px;height:122px;"><a href="/wps/find/homepage.cws_home"><img src="/authored_framework/images/logo_tree.gif" width="178" height="121" border="0" alt="Go to Elsevier home page" /></a></td>
		</tr>
	</table>

<!-- end of banner -->
<div id="FLYParent"><div class="themeHeader"></div>




<table style="width:100%;" cellpadding="0px" cellspacing="0px"><tr><td valign="top"></td><td width="100%" height="100%" valign="top"><a name="wpsMainContent"></a><div id="mainContent"><table border="0" width="100%" cellpadding="0" cellspacing="0" align="center"><tr height="100%"><td valign="top" width="155"><table border="0" width="100%" cellpadding="0" cellspacing="0" align="center"><tr><td width="100%" valign="top"><a name="7_KL9G95420OKE4025H5GIB73003"></a><div class="wpsPortletBody"><script language="JavaScript">
<!--
var selectedSubitem = -1
//-->
</script>

<table cellspacing="0" cellpadding="0" border="0" width="155">
	<tr>
		<td><img src="/authored_framework/images/empty.gif" width="155" height="19" border="0" alt=""></td>
	</tr>
</table>

<table cellpadding="0" cellspacing="0" border="0">
<tr>
<td width="1"><img src="/authored_framework/images/empty.gif" width="1" height="1" border="0" alt=""></td>
<td>

	<table cellpadding="0" cellspacing="0" border="0" class="tableTextHeader" onclick="window.location.href='/wps/find/subject_area_browse.cws_home?collapseAll=y&sh1State=0&allParents=y'" onMouseOver="headerOver('Products')" onMouseOut="headerOut()">
		<tr>
			<td class="textHeader" colspan="3"><img src="/authored_framework/images/empty.gif" height="2" width="1" border="0" alt=""></a></td>
		</tr>
		<tr>
			<td class="textHeader" width="5"><img src="/authored_framework/images/empty.gif" height="1" width="5" border="0" alt=""></a></td>
			<td class="textHeader"><a href='/wps/find/subject_area_browse.cws_home?collapseAll=y&sh1State=0&allParents=y'>Products</a></td>
			<td class="textHeader" width="5"><img src="/authored_framework/images/empty.gif" height="1" width="5" border="0" alt=""></a></td>
		</tr>
		<tr>
			<td class="textHeader" colspan="3"><img src="/authored_framework/images/empty.gif" height="2" width="1" border="0" alt=""></a></td>
		</tr>
	</table>
	<table cellpadding="0" cellspacing="0" border="0">		<tr>
			<td class="item" height="14" width="153">
				<table cellpadding="0" cellspacing="0" border="0">
					<tr>
						<td><img src="/authored_framework/images/empty.gif" width="5" height="1" border="0" alt=""></td>
						<td class="itemText">Browse by subject</td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="itemLine"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem2" class="subItem" height="14" onclick='window.location.href="/wps/find/subject_area_browse.cws_home?collapseAll=y&sh1State=0&allParents=y"' onmouseover="subItemOver2(this, 2, 'All subjects', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/subject_area_browse.cws_home?collapseAll=y&sh1State=0&allParents=y'>All subjects</a></td>
						<td width="6"><img id="arrow2" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line2"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem3" class="subItem" height="14" onclick='window.location.href="/wps/find/subject_area_browse.cws_home/?sh1State=-null-SAR-SAA-SAC-SAD-SAF-SA1-SAI-SAJ-SAK-SAQ-SAP-SAB-SAE-SAL-SAN-SAO-SAG-SAH-SAM-null&sh2State=&SH0Only=PS"' onmouseover="subItemOver2(this, 3, 'Physical sciences', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/subject_area_browse.cws_home/?sh1State=-null-SAR-SAA-SAC-SAD-SAF-SA1-SAI-SAJ-SAK-SAQ-SAP-SAB-SAE-SAL-SAN-SAO-SAG-SAH-SAM-null&sh2State=&SH0Only=PS'>Physical sciences</a></td>
						<td width="6"><img id="arrow3" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line3"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem4" class="subItem" height="14" onclick='window.location.href="/wps/find/subject_area_browse.cws_home/?sh1State=-null-SAR-SAA-SAC-SAD-SAF-SA1-SAI-SAJ-SAK-SAQ-SAP-SAB-SAE-SAL-SAN-SAO-SAG-SAH-SAM-null&sh2State=&SH0Only=HS"' onmouseover="subItemOver2(this, 4, 'Health sciences', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/subject_area_browse.cws_home/?sh1State=-null-SAR-SAA-SAC-SAD-SAF-SA1-SAI-SAJ-SAK-SAQ-SAP-SAB-SAE-SAL-SAN-SAO-SAG-SAH-SAM-null&sh2State=&SH0Only=HS'>Health sciences</a></td>
						<td width="6"><img id="arrow4" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line4"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem5" class="subItem" height="14" onclick='window.location.href="/wps/find/subject_area_browse.cws_home/?sh1State=-null-SAR-SAA-SAC-SAD-SAF-SA1-SAI-SAJ-SAK-SAQ-SAP-SAB-SAE-SAL-SAN-SAO-SAG-SAH-SAM-null&sh2State=&SH0Only=SS"' onmouseover="subItemOver2(this, 5, 'Social sciences', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/subject_area_browse.cws_home/?sh1State=-null-SAR-SAA-SAC-SAD-SAF-SA1-SAI-SAJ-SAK-SAQ-SAP-SAB-SAE-SAL-SAN-SAO-SAG-SAH-SAM-null&sh2State=&SH0Only=SS'>Social sciences</a></td>
						<td width="6"><img id="arrow5" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line5"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem6" class="subItem" height="14" onclick='window.location.href="/wps/find/subject_area_browse.cws_home/?sh1State=-null-SAR-SAA-SAC-SAD-SAF-SA1-SAI-SAJ-SAK-SAQ-SAP-SAB-SAE-SAL-SAN-SAO-SAG-SAH-SAM-null&sh2State=&SH0Only=LS"' onmouseover="subItemOver2(this, 6, 'Life sciences', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/subject_area_browse.cws_home/?sh1State=-null-SAR-SAA-SAC-SAD-SAF-SA1-SAI-SAJ-SAK-SAQ-SAP-SAB-SAE-SAL-SAN-SAO-SAG-SAH-SAM-null&sh2State=&SH0Only=LS'>Life sciences</a></td>
						<td width="6"><img id="arrow6" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line6"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td class="item" height="14" width="153">
				<table cellpadding="0" cellspacing="0" border="0">
					<tr>
						<td><img src="/authored_framework/images/empty.gif" width="5" height="1" border="0" alt=""></td>
						<td class="itemText">Browse by product type</td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="itemLine"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem8" class="subItem" height="14" onclick='window.location.href="/wps/find/books_browse.cws_home"' onmouseover="subItemOver2(this, 8, 'Books', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/books_browse.cws_home'>Books</a></td>
						<td width="6"><img id="arrow8" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line8"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem9" class="subItem" height="14" onclick='window.location.href="/wps/find/journal_browse.cws_home"' onmouseover="subItemOver2(this, 9, 'Journals', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/journal_browse.cws_home'>Journals</a></td>
						<td width="6"><img id="arrow9" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line9"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem10" class="subItem" height="14" onclick='window.location.href="/wps/find/electronic_browse.cws_home"' onmouseover="subItemOver2(this, 10, 'Electronic products', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/electronic_browse.cws_home'>Electronic products</a></td>
						<td width="6"><img id="arrow10" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line10"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem11" class="subItem" height="14" onclick='window.location.href="/wps/find/bibliographic_browse.cws_home"' onmouseover="subItemOver2(this, 11, 'Bibliographic databases', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/bibliographic_browse.cws_home'>Bibliographic databases</a></td>
						<td width="6"><img id="arrow11" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line11"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem12" class="subItem" height="14" onclick='window.location.href="/wps/find/newsletter_browse.cws_home"' onmouseover="subItemOver2(this, 12, 'Newsletters and other product types', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/newsletter_browse.cws_home'>Newsletters and other product types</a></td>
						<td width="6"><img id="arrow12" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line12"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem13" class="subItem" height="14" onclick='window.location.href="/wps/find/all_products_browse.cws_home"' onmouseover="subItemOver2(this, 13, 'All product types', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/all_products_browse.cws_home'>All product types</a></td>
						<td width="6"><img id="arrow13" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line13"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem14" class="itemLink" height="14" onclick='window.location.href="/wps/find/advproductsearch.cws_home?action=product_search&search=no"' onmouseover="subItemOver2(this, 14, 'Advanced product search ', '#336699')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="5"><img src="/authored_framework/images/empty.gif" width="5" height="1" border="0" alt=""></td>
						<td class="itemLinkText"><a href='/wps/find/advproductsearch.cws_home?action=product_search&search=no'>Advanced product search </a></td>
						<td width="6"><img id="arrow14" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line14"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td class="item" height="14" width="153">
				<table cellpadding="0" cellspacing="0" border="0">
					<tr>
						<td><img src="/authored_framework/images/empty.gif" width="5" height="1" border="0" alt=""></td>
						<td class="itemText">Catalogs</td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="itemLine"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem17" class="subItem" height="14" onclick='window.location.href="/wps/find/subscriptionpricelist.cws_home/subscriptionpricelist/description"' onmouseover="subItemOver2(this, 17, 'Subscription price list', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/subscriptionpricelist.cws_home/subscriptionpricelist/description'>Subscription price list</a></td>
						<td width="6"><img id="arrow17" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line17"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td class="item" height="14" width="153">
				<table cellpadding="0" cellspacing="0" border="0">
					<tr>
						<td><img src="/authored_framework/images/empty.gif" width="5" height="1" border="0" alt=""></td>
						<td class="itemText">Product support</td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="itemLine"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem19" class="subItem" height="14" onclick='window.location.href="/wps/find/productsupportfaq.cws_home/overview"' onmouseover="subItemOver2(this, 19, 'Help and FAQ', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/productsupportfaq.cws_home/overview'>Help and FAQ</a></td>
						<td width="6"><img id="arrow19" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line19"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td id="subItem20" class="subItem" height="14" onclick='window.location.href="/wps/find/productcontact.cws_home/regional"' onmouseover="subItemOver2(this, 20, 'Support & sales offices', '#6699CC')" onmouseout="subItemOut2(this)">			
				<table cellpadding="0" cellspacing="0" border="0" width="153">
					<tr>
						<td width="10"><img src="/authored_framework/images/empty.gif" width="10" height="1" border="0" alt=""></td>
						<td class="subItemText"><a href='/wps/find/productcontact.cws_home/regional'>Support & sales offices</a></td>
						<td width="6"><img id="arrow20" src="/authored_framework/images/empty.gif" width="3" height="7" border="0" alt=""></td>
					</tr>
				</table>
			</td>
		</tr>
		<tr>
			<td class="subItemLine" id="line20"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
		<tr>
			<td class="subItemLineBottom"><img src="/authored_framework/images/empty.gif" width="153" height="1" border="0" alt=""></td>
		</tr>
	</table>
	<table cellpadding="0" cellspacing="0" border="0">
		<tr>
			<td><img src="/authored_framework/images/empty.gif" height="8" width="1" border="0" alt=""></a></td>
		</tr>
	</table>
	<table cellpadding="0" cellspacing="0" border="0" class="tableTextHeader" onclick="window.location.href='/wps/find/supportfaq.cws_home/overview'" onMouseOver="headerOver('Support &amp; contact')" onMouseOut="headerOut()">
		<tr>
			<td class="textHeader" colspan="3"><img src="/authored_framework/images/empty.gif" height="2" width="1" border="0" alt=""></a></td>
		</tr>
		<tr>
			<td class="textHeader" width="5"><img src="/authored_framework/images/empty.gif" height="1" width="5" border="0" alt=""></a></td>
			<td class="textHeader"><a href='/wps/find/supportfaq.cws_home/overview'>Support &amp; contact</a></td>
			<td class="textHeader" width="5"><img src="/authored_framework/images/empty.gif" height="1" width="5" border="0" alt=""></a></td>
		</tr>
		<tr>
			<td class="textHeader" colspan="3"><img src="/authored_framework/images/empty.gif" height="2" width="1" border="0" alt=""></a></td>
		</tr>
	</table>
	<table cellpadding="0" cellspacing="0" border="0"><tr><td></td></tr>	</table>
	<table cellpadding="0" cellspacing="0" border="0">
		<tr>
			<td><img src="/authored_framework/images/empty.gif" height="8" width="1" border="0" alt=""></a></td>
		</tr>
	</table>
	<table cellpadding="0" cellspacing="0" border="0" class="tableTextHeader" onclick="window.location.href='/wps/find/intro.cws_home/ataglance'" onMouseOver="headerOver('About Elsevier')" onMouseOut="headerOut()">
		<tr>
			<td class="textHeader" colspan="3"><img src="/authored_framework/images/empty.gif" height="2" width="1" border="0" alt=""></a></td>
		</tr>
		<tr>
			<td class="textHeader" width="5"><img src="/authored_framework/images/empty.gif" height="1" width="5" border="0" alt=""></a></td>
			<td class="textHeader"><a href='/wps/find/intro.cws_home/ataglance'>About Elsevier</a></td>
			<td class="textHeader" width="5"><img src="/authored_framework/images/empty.gif" height="1" width="5" border="0" alt=""></a></td>
		</tr>
		<tr>
			<td class="textHeader" colspan="3"><img src="/authored_framework/images/empty.gif" height="2" width="1" border="0" alt=""></a></td>
		</tr>
	</table>
	<table cellpadding="0" cellspacing="0" border="0"><tr><td></td></tr>	</table>
	<table cellpadding="0" cellspacing="0" border="0">
		<tr>
			<td><img src="/authored_framework/images/empty.gif" height="8" width="1" border="0" alt=""></a></td>
		</tr>
	</table>
	<table cellpadding="0" cellspacing="0" border="0" class="tableTextHeader" onclick="window.location.href='/wps/find/simple_content.cws_home/pagenotfound?navopenmenu=3'" onMouseOver="headerOver('Select your view')" onMouseOut="headerOut()">
		<tr>
			<td class="textHeader" colspan="3"><img src="/authored_framework/images/empty.gif" height="2" width="1" border="0" alt=""></a></td>
		</tr>
		<tr>
			<td class="textHeader" width="5"><img src="/authored_framework/images/empty.gif" height="1" width="5" border="0" alt=""></a></td>
			<td class="textHeader"><a href='/wps/find/simple_content.cws_home/pagenotfound?navopenmenu=3'>Select your view</a></td>
			<td class="textHeader" width="5"><img src="/authored_framework/images/empty.gif" height="1" width="5" border="0" alt=""></a></td>
		</tr>
		<tr>
			<td class="textHeader" colspan="3"><img src="/authored_framework/images/empty.gif" height="2" width="1" border="0" alt=""></a></td>
		</tr>
	</table>
	<table cellpadding="0" cellspacing="0" border="0"><tr><td></td></tr>	</table>
	<table cellpadding="0" cellspacing="0" border="0">
		<tr>
			<td><img src="/authored_framework/images/empty.gif" height="8" width="1" border="0" alt=""></a></td>
		</tr>
	</table>


</td>
</tr>
</table>



</div></td></tr></table></td><td valign="top" ><table border="0" width="100%" cellpadding="0" cellspacing="0" align="center"><tr><td width="100%" valign="top"><a name="7_KL9G95420OKE4025H5GIB730G0"></a><div class="wpsPortletBody"><!DOCTYPE HTML PUBLIC "-//W3C//DTD HTML 4.01 Transitional//EN">








<HTML>
<HEAD>

<META http-equiv="Content-Type" content="text/html; charset=ISO-8859-1">
<META name="GENERATOR" content="IBM WebSphere Studio">
<TITLE>SiteStat.jsp</TITLE>
</HEAD>

<BODY>

<!-- Begin Sitestat4 code -->
<script language="JavaScript1.1">
<!--
function sitestat(ns_l){ns_l+="&ns__t="+(new Date()).getTime();ns_pixelUrl=ns_l;
ns_0=document.referrer;
ns_0=(ns_0.lastIndexOf("/")==ns_0.length-1)?ns_0.substring(ns_0.lastIndexOf("/"),0):ns_0;
if(ns_0.length>0)ns_l+="&ns_referrer="+escape(ns_0);
if(document.images){ns_1=new Image();ns_1.src=ns_l;}else
document.write("<img src="+ns_l+" width='1' height='1'>");}
sitestat("http://nl.sitestat.com/elsevier/elsevier-com/s?general_info.simple_content.pagenotfound&category=cws_home");
//-->
</script>
<noscript>
<img src="http://nl.sitestat.com/elsevier/elsevier-com/s?general_info.simple_content.pagenotfound&category=cws_home" width="1" height="1">
</noscript>
<!-- End Sitestat4 code -->

</BODY>
</HTML>
</div></td></tr><tr><td width="100%" valign="top"><a name="7_KL9G95420OKE4025H5GIB730G2"></a><div class="wpsPortletBody"><?xml-stylesheet type="text/xsl">
<html>
    <head>
        <META http-equiv="Content-Type" content="text/html; charset=UTF-8">
        <LINK TYPE="text/css" REL="STYLESHEET" HREF="/framework_include/css/elsevier.css">
        <LINK TYPE="text/css" REL="STYLESHEET" HREF="/framework_include/css/elsevier2.css">
        <META HTTP-EQUIV="Content-Type" CONTENT="text/html;charset=UTF-8">
    </head>
    <body>
        <table width="100%" cellspacing="0" cellpadding="0" border="0">
            <tr>
                <td style="background-color:#ffffff;"><img src="/framework_images/empty.gif" height="1" border="0" alt=""></td><td style="background-color:#ffffff;"><img src="/framework_images/empty.gif" height="1" border="0" alt=""></td><td style="width:2px;background-color:#ffffff;"><img width="2" src="/framework_images/empty.gif" height="1" border="0" alt=""></td>
            </tr>
            <tr>
                <td valign="top" style="background-color:#ffffff;">
                    <table width="100%" cellspacing="0" cellpadding="0" border="0">
                        <tr>
                            <td colspan="3"><a name="top"></a><img width="1" src="/framework_images/empty.gif" height="20" border="0" alt=""></td>
                        </tr>
                        <tr>
                            <td style="width:25px;"><img width="25" src="/framework_images/empty.gif" height="1" border="0" alt=""></td><td><img src="/framework_home/images/headers/pagenotfound.gif" alt="Page not found at the Elsevier Corporate Website"><br>
                            </td><td style="width:25px;"><img width="25" src="/framework_images/empty.gif" height="1" border="0" alt=""></td>
                        </tr>
                        <tr>
                            <td style="width:25px;"><img width="25" src="/framework_images/empty.gif" height="1" border="0" alt=""></td><td style="background-color:#E3E3E3"><img width="1" src="/framework_images/empty.gif" height="1" border="0" alt=""></td><td style="width:25px;"><img width="25" src="/framework_images/empty.gif" height="1" border="0" alt=""></td>
                        </tr>
                        <tr>
                            <td colspan="3"><img width="1" src="/framework_images/empty.gif" height="10" border="0" alt=""></td>
                        </tr>
                        <tr>
                            <td style="width:25px;"><img width="25" src="/framework_images/empty.gif" height="1" border="0" alt=""></td><td class="verdana11DarkGrey">
                                <table width="100%" cellspacing="0" cellpadding="0" border="0">
                                    <tr>
                                        <td class="verdana11DarkGrey">
                                            <P>The page you are looking for might have been (re)moved or is currently unavailable.</P>

                                            <P>Suggestions:</P>

                                            <UL>

                                                <LI>Please review your URL in the Address bar, or</LI>

                                                <LI>Click the Refresh button in your local browser, or</LI>

                                                <LI>Go to the <a href="/wps/find/homepage.cws_home"><FONT color="#FF6600">Homepage</FONT></a>, or</LI>

                                                <LI>Go to Previous Page to verify your action, or</LI>

                                                <LI>Go to the <a href="/wps/find/sitemap.cws_home/sitemap"><FONT color="#FF6600">Site map</FONT></a>, or</LI>

                                                <LI>Go to Search Box on top of this page for a search</LI>

                                            </UL>

                                            <P></P>
                                        </td>
                                    </tr>
                                </table>
                            </td><td style="width:25px;"><img width="25" src="/framework_images/empty.gif" height="1" border="0" alt=""></td>
                        </tr>
                        <tr>
                            <td style="width:25px;"><img width="25" src="/framework_images/empty.gif" height="1" border="0" alt=""></td><td align="right"><img width="19" src="/framework_images/empty.gif" height="1" border="0" alt=""></td><td style="width:25px;"><img width="25" src="/framework_images/empty.gif" height="1" border="0" alt=""></td>
                        </tr>
                        <tr>
                            <td colspan="3"><img width="1" src="/framework_images/empty.gif" height="30" border="0" alt=""></td>
                        </tr>
                        <tr>
                            <td colspan="3"><img width="1" src="/framework_images/empty.gif" height="25" border="0" alt=""></td>
                        </tr>
                    </table>
                </td><td style="width:2px;background-color:#ffffff;"><img width="2" src="/framework_images/empty.gif" height="1" border="0" alt=""></td>
            </tr>
        </table>
    </body>
</html>
</div></td></tr></table></td></tr></table></div></td></tr></table>
<!-- Start of page functions bar -->




<script language="JavaScript" type="text/javascript">
<!--
function openPrinterFriendlyPage() {
	if (location.href.indexOf("/wps/find/") > -1) {
		var urlToSplit = location.href		
		var qryStr = ""
		if (location.href.indexOf("?") > -1) {
			//qryStr = location.href.substring(location.href.indexOf("?"))
			urlToSplit = location.href.substring(0, location.href.indexOf("?"))
		}
		var pieces = urlToSplit.split("/")
		var prvPiece = ""
		var printUrl = ""
		/***************Temp Fix for cws_home print theme ***************/
		var home = ""
		var placeName = ""
		/***************End of Temp Fix for cws_home print theme ***************/
		
		for (var i = 0; i < pieces.length; i++) {
			if (i > 0) {
				printUrl += "/"
			}
			if (prvPiece == "find") {
				if (pieces[i].indexOf(".") > -1) {
					dotPos = pieces[i].indexOf(".")
					if (pieces[i].substring(dotPos).indexOf("cws_home") > -1) {
						home = "cws_home"
					}else{
						home = "cws_home"
					}
					printUrl += pieces[i].substring(0, dotPos) + ".print"
				} else {
					alert("This page does not have a printer-friendly version")
					return
				}
			} else {
				printUrl += pieces[i]
			}
			prvPiece = pieces[i]
		}

		

		var isTheirParams = "false"
		var qpString = ""		
		if(qpString.length > 0) {
			isTheirParams = "true"
		}
		
		qryStr = "?avoidEmail=true"

		if (home != "") {
		
			qryStr += "&" + "printHome=" + home			
			home = ""
		}
		
		if(isTheirParams == "true") {			
			qryStr += "&" + qpString
		}

		
				
		printUrl += qryStr
		//alert("The URL:" + printUrl + ":")
		window.open(printUrl, "print", "height=470,left=20,menubar=1,scrollbars=1,status=0,top=20,resizable=1,width=670");
	} else {
		alert("This page does not have a printer-friendly version")
	}
}
// --> 
</script>

<table cellpadding="0" cellspacing="0" border="0" width="100%">
<tr>
<td style="width:1px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="1" height="1" border="0" alt="" /></td>
<td style="width:154px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="154" height="1" border="0" alt="" /></td>
<td style="background-color:#ffffff;" valign="top">
	<table cellpadding="0" cellspacing="0" border="0" width="100%">
	<tr>
	<td colspan="3"><img src="/authored_framework/images/empty.gif" width="1" height="15" border="0" alt="" /></td>
	</tr>
	<tr>
	<td style="width:25px;"><img src="/authored_framework/images/empty.gif" width="25" height="1" border="0" alt="" /></td>
	<td align="right">
		<table cellpadding="0" cellspacing="0" border="0">
		<tr>
		<td>
		<a href="javascript:openPrinterFriendlyPage()"><img src="/authored_framework/images/buttons/print.gif" width="20" height="19" border="0" alt="Printer-friendly version" /></a>
		</td>
		<td>
		&nbsp;&nbsp;<a class="verdana10DarkGrey" href="javascript:openPrinterFriendlyPage()">Printer-friendly version</a>
		</td>
		</tr>
		</table>
	</td>
	<td style="width:25px;"><img src="/authored_framework/images/empty.gif" width="25" height="1" border="0" alt="" /></td>
	</tr>
	</table>
</td>
<td style="width:157px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="157" height="1" border="0" alt="" /></td>
<td style="width:2px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="2" height="1" border="0" alt="" /></td>
</tr>
</table>

<table cellpadding="0" cellspacing="0" border="0" width="100%">
<tr>
<td style="height:30px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="1" height="30" border="0" alt="" /></td>
</tr>
</table>

<!-- End of page functions bar -->

<!-- Start of bottom bar -->

<table cellpadding="0" cellspacing="0" border="0" width="100%">
<tr>
<td style="width:1px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="1" height="1" border="0" alt="" /></td>
<td style="width:154px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="154" height="1" border="0" alt="" /></td>
<td style="background-color:#FF9933;height:27px;">
<table cellpadding="0" cellspacing="0" border="0" width="100%">
<tr>
<td style="width:25px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="25" height="1" border="0" alt="" /></td>
<td style="background-color:#ffffff;" align="right"><img src="/authored_framework/images/empty.gif" width="1" height="10" border="0" alt="" /></td>
</tr>
<tr>
<td style="width:25px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="25" height="1" border="0" alt="" /></td>
<td style="background-color:#FF9933;height:17px;" align="right">
<table cellpadding="1" cellspacing="0" border="0" width="100%">
<tr>
<td align="left" class="verdana10White">&nbsp;<a href="/wps/find/homepage.cws_home">Home</a> | 
<a href="/wps/find/sitemap.cws_home/sitemap">Site map</a> | 
<a href="/wps/find/privacypolicy.cws_home/privacypolicy">Privacy policy</a> | 
<a href="/wps/find/termsconditions.cws_home/termsconditions">Terms and Conditions</a> | 
<a href="/wps/find/feedbackform.cws_home">Feedback</a> | 
<nobr>A <a href="http://www.reed-elsevier.com" target="reed_elsevier">Reed Elsevier</a> company</nobr></td>
<td align="right" style="width:5px;"><img src="/authored_framework/images/empty.gif" width="5" height="1" border="0" alt="" /></td>
</tr>
<tr><td bgcolor="#ffffff" colspan="2"><img src="/authored_framework/images/empty.gif" width="1" height="1" /></td></tr>
<tr>
<td align="left" colspan="2" bgcolor="#ffffff" style="font-size: 10px;">
&nbsp;Copyright &copy; 2008 <a href="/wps/find/homepage.cws_home" style="FONT-SIZE: 10px; CURSOR: default; COLOR: #ff9933; FONT-FAMILY: verdana, arial, sans-serif;">Elsevier B.V.</a> All rights reserved.
</td>
</tr>
</table>
</td>
</tr>
</table>
</td>
<td style="width:2px;background-color:#ffffff;"><img src="/authored_framework/images/empty.gif" width="2" height="1" border="0" alt="" /></td>
</tr>
</table>

<!-- End of bottom bar -->
</div>



</body></html>
